Self-Monitoring Navigation Agent via Auxiliary Progress Estimation

The Vision-and-Language Navigation (VLN) task entails an agent following navigational instruction in photo-realistic unknown environments. This challenging task demands that the agent be aware of which instruction was completed, which instruction is needed next, which way to go, and its navigation progress towards the goal. In this paper, we introduce a self-monitoring agent with two complementary components: (1) visual-textual co-grounding module to locate the instruction completed in the past, the instruction required for the next action, and the next moving direction from surrounding images and (2) progress monitor to ensure the grounded instruction correctly reflects the navigation progress. We test our self-monitoring agent on a standard benchmark and analyze our proposed approach through a series of ablation studies that elucidate the contributions of the primary components. Using our proposed method, we set the new state of the art by a significant margin (8% absolute increase in success rate on the unseen test set). Code is available at https://github.com/chihyaoma/selfmonitoring-agent .

==> sections/messy.tex <==
\section*{Paper progress}
\textbf{Review}. Any comments and suggestions are welcome. 
You can leave comments via Overleaf built-in function, use \textit{textcolor} command with different colors, or directly revise the paper (\textbf{preferred}).
If you decided to revise the paper directly, \textit{track-changes} (Ab Review on top right corner) should have already be enabled for you. In this way, I can keep track of what changes have been made by all of you. 
I will check out the changes constantly everyday until we submit the paper. 
Thank you all for your great help and valuable inputs!

The following sections are ready for revise:
\begin{itemize}
    \item[$\square$] Introduction
    \item[$\square$] Method
    \item[$\square$] Experiments
\end{itemize}

The following parts are currently in the process:
\begin{itemize}
    \item[$\square$] Figures and revising the whole paper except related work section
\end{itemize}

Notes:
\begin{itemize}
% 	\item Robot navigation is important to motivate ICLR reviewers
% 	\item robot navigation two different setting: given map, without map 
% 	\item given goal/destination, given instruction 
% 	\item Figure 1 demonstrates VLN task and demonstrates high-level concept
% 	\item test submission name: self-aware co-grounded model
	\item Jiasen: propose an evaluation metric for ctx attention.
	\item Jianwei: minor concerns: Similar to value function in A2C (can mention as "in the similar spirits with"); why not restrict attention on instruction to different parts.
	\item Caiming: in the second paragraph of intro, what is the previous navigation task?
\end{itemize}

==> tables/ablation_instr.tex <==

\begin{table}[b]
\centering
\small
\tabcolsep=0.13cm
% \caption{
%     Ablation study on using instruction or not when choosing the next action. 
%     We implemented the model from Speaker-Follower~(\cite{fried2018speaker}) with panoramic action space as baseline model.
%     \footnote{Note that our results for this baseline are slightly higher on val-unseen and slightly lower on val-seen than those reported, due to differences in implementation details and hyper-parameter choices.}
%     }
\caption[Caption for LOF]{\textcolor{red}{(To be removed)} Ablation study on using instruction or not when choosing the next action. 
    % We implemented the model from Speaker-Follower~(\cite{fried2018speaker}) with panoramic action space as baseline\protect\footnotemark.
    }
\label{table:ablation-study-instruction}
\begin{tabular}{ccccccccc}
\Xhline{2\arrayrulewidth}
                                                                      & \multicolumn{2}{c}{Choose action with} & \multicolumn{3}{c}{Validation-Seen} & \multicolumn{3}{c}{Validation-Unseen} \\ \cline{4-9} 
                                                                      & instruction & $h_t$ & NE $\downarrow$        & SR $\uparrow$       & OSR $\uparrow$        & NE $\downarrow$        & SR $\uparrow$         & OSR $\uparrow$        \\ \hline
\begin{tabular}[c]{@{}c@{}}Baseline\tnote{*}\\ (Speaker-Follower)\end{tabular} & \checkmark      &     & 4.36     & 0.54           & 0.68          & 7.22    & 0.27           & 0.39 \\ \hline
Baseline                                                              &             & \checkmark    & 5.35           & 0.46           & 0.60           & 6.67            & 0.31           & 0.43            \\
Baseline                                                              & \checkmark           & \checkmark    & 4.65           & 0.52          & 0.66           & 6.84           & 0.32           & 0.43           \\ \Xhline{2\arrayrulewidth}
\end{tabular}
\end{table}

% \footnotetext{Note that our results for this baseline are slightly higher on val-seen and slightly lower on val-unseen than those reported, due to differences in hyper-parameter choices. We thank the authors for communicating with us and providing details of the implementation.}


% \begin{table}[tb]
% \centering
% \small
% \tabcolsep=0.13cm
% \caption{
%     Ablation study on using instruction or not when choosing the next action. 
%     We implemented the model from Speaker-Follower~(\cite{fried2018speaker}) with panoramic action space as baseline model.
%     }
% \label{table:ablation-study-instruction-1}
% \begin{threeparttable}
% \begin{tabular}{ccccccccc}
% \Xhline{2\arrayrulewidth}

%                                                                       & \multicolumn{2}{c}{Choose action with} & \multicolumn{3}{c}{Validation-Seen} & \multicolumn{3}{c}{Validation-Unseen} \\ \cline{4-9} 
%                                                                       & instruction & $h_t$ & NE $\downarrow$        & SR $\uparrow$       & OSR $\uparrow$        & NE $\downarrow$        & SR $\uparrow$         & OSR $\uparrow$        \\ \hline
% \begin{tabular}[c]{@{}c@{}}Baseline\tnote{*}\\ (Speaker-Follower)\end{tabular} & \checkmark           &      &            &           &            &            &            &             \\
% Baseline                                                              &             & \checkmark    &            &           &            &            &            &             \\
% Baseline                                                              & \checkmark           & \checkmark    &            &           &            &            &            &            \\ \Xhline{2\arrayrulewidth}
% \end{tabular}
% \begin{tablenotes}\footnotesize
% \item[*] This is our baseline implementation of Speaker-Follower~(\cite{fried2018speaker}). 
% Note that our results for this baseline are slightly higher on val-unseen and slightly lower on val-seen than
% those reported, due to differences in implementation details and hyper-parameter choices.
% \end{tablenotes}
% \end{threeparttable}
% \end{table}


==> tables/ablation_study.tex <==
% ====================================================================================
% \begin{table}[t]
% \centering
% \small
% \tabcolsep=0.13cm
% \caption{
%     Ablation study showing the effect of each proposed method compared to the prior arts. All methods are using panoramic action space.
%     \textcolor{red}{add full speaker-follower model with data augmentation?}
% }
% \label{table:ablation-study}
% % \begin{tabular}{cccccccccc}
% % \Xhline{2\arrayrulewidth}
% %                                       & Data                 & Pragmatic            & Beam                 & \multicolumn{3}{c}{Validation-Seen}                                & \multicolumn{3}{c}{Validation-Unseen}                              \\ \cline{5-10} 
% %                                       & Augmentation         & Inference            & Search               & NE                   & SR                   & OSR                  & NE                   & SR                   & OSR                  \\ \hline
% % Speaker-Follower                       &                      &                      &                      & 4.86                 & 52.1                 & 63.3                 & 7.07                 & 31.2                 & 41.3                 \\
% % Ours                                   & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\ \hline
% % \multirow{2}{*}{Speaker-Follower}      &                      & \checkmark            & \checkmark            & 3.88                 & 63.3                 & 71.0                 & 5.24                 & 49.5                 & 63.4                 \\
% %                                       & \checkmark            & \checkmark            & \checkmark            & 3.08                 & 70.1                 & 78.3                 & 4.83                 & 54.6                 & 65.2                 \\
% % \multirow{2}{*}{Ours (self-awareness)} &                      &                      &                      & 3.72                 & 63.3                 & 74.5                 & 5.98                 & 43.8                 & 57.5                 \\
% %                                       &                      &                      & \checkmark            & 3.23                 & 69.7                 & 77.6                 & 5.04                 & 57.1                 & 69.6                 \\ \Xhline{2\arrayrulewidth}
% % \end{tabular}
% \begin{tabular}{cccccccccc}
% \Xhline{2\arrayrulewidth}
%                                       & Pragmatic            & Beam                 & Panoramic & \multicolumn{3}{c}{Validation-Seen}                                & \multicolumn{3}{c}{Validation-Unseen}                              \\ \cline{5-10} 
%                                       & Inference            & Search               & Space     & NE                   & SR                   & OSR                  & NE                   & SR                   & OSR                  \\ \hline
% Speaker-Follower                       &                      &                      & \checkmark & 4.86                 & 52.1                 & 63.3                 & 7.07                 & 31.2                 & 41.3                 \\
% Ours                                   & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \checkmark & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\ \hline
% Speaker-Follower                       & \checkmark            & \checkmark            & \checkmark & 3.88                 & 63.3                 & 71.0                 & 5.24                 & 49.5                 & 63.4                 \\
% \multirow{2}{*}{Ours (self-awareness)} &                      &                      & \checkmark & 3.72                 & 63.3                 & 74.5                 & 5.98                 & 43.8                 & 57.5                 \\
%                                       &                      & \checkmark            & \checkmark & \textbf{3.23}        & \textbf{69.7}        & \textbf{77.6}        & \textbf{5.04}        & \textbf{57.1}        & \textbf{69.6}        \\ \Xhline{2\arrayrulewidth}
% \end{tabular}
% \end{table}
% ====================================================================================

% ====================================================================================
% \begin{table}[t]
% \centering
% \small
% \tabcolsep=0.13cm
% \caption{
%     Ablation study showing the effect of each proposed method compared to the prior arts. All methods are using panoramic action space.
%     \textcolor{red}{remove full speaker-follower model with data augmentation?}
% }
% \label{table:ablation-study-2}
% \begin{tabular}{cccccccccc}
% \Xhline{2\arrayrulewidth}
%                                       & Data                 & Pragmatic            & Beam                 & \multicolumn{3}{c}{Validation-Seen}                                & \multicolumn{3}{c}{Validation-Unseen}                              \\ \cline{5-10} 
%                                       & Augmentation         & Inference            & Search               & NE                   & SR                   & OSR                  & NE                   & SR                   & OSR                  \\ \hline
% Speaker-Follower                       &                      &                      &                      & 4.86                 & 52.1                 & 63.3                 & 7.07                 & 31.2                 & 41.3                 \\
% % Ours                                   & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{3.73} & \multicolumn{1}{l}{64.1} & \multicolumn{1}{l}{75.6} & \multicolumn{1}{l}{6.01} & \multicolumn{1}{l}{43.2} & \multicolumn{1}{l}{55.3} \\ \hline
% % Ours                                   & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{3.82} & \multicolumn{1}{l}{64.2} & \multicolumn{1}{l}{75.9} & \multicolumn{1}{l}{6.04} & \multicolumn{1}{l}{41.9} & \multicolumn{1}{l}{57.3} \\ \hline
% Ours                                   & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\ \hline
% \multirow{2}{*}{Speaker-Follower}      &                      & \checkmark            & \checkmark            & 3.88                 & 63.3                 & 71.0                 & 5.24                 & 49.5                 & 63.4                 \\
%                                       & \checkmark            & \checkmark            & \checkmark            & \textbf{3.08}                 & \textbf{70.1}                 & \textbf{78.3}                 & \textbf{4.83}                 & 54.6                 & 65.2                 \\
% \multirow{2}{*}{Ours (self-awareness)} &                      &                      &                      & 3.72                 & 63.3                 & 74.5                 & 5.98                 & 43.8                 & 57.5                 \\
%                                       &                      &                      & \checkmark            & 3.23                 & 69.7                 & 77.6                 & 5.04                 & \textbf{57.1}                 & \textbf{69.6}                 \\ \Xhline{2\arrayrulewidth}
% \end{tabular}
% \end{table}
% ====================================================================================

% ====================================================================================
% \begin{table}[t]
% \centering
% \small
% \tabcolsep=0.13cm
% \caption{
%     Ablation study showing the effect of each proposed method compared to the prior arts. All methods are using panoramic action space.
%     \textcolor{red}{remove full speaker-follower model with data augmentation?}
% }
% \label{table:ablation-study-3}
% \begin{tabular}{cccccccccc}
% \Xhline{2\arrayrulewidth}
%                                       & Data                 & Pragmatic            & Beam                 & \multicolumn{3}{c}{Validation-Seen}                                & \multicolumn{3}{c}{Validation-Unseen}                              \\ \cline{5-10} 
%                                       & Augmentation         & Inference            & Search               & NE                   & SR                   & OSR                  & NE                   & SR                   & OSR                  \\ \hline
% Speaker-Follower                       &                      &                      &                      & 4.86                 & 0.52                 & 0.63                 & 7.07                 & 0.31                 & 0.41                \\
% % Ours                                   & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{3.73} & \multicolumn{1}{l}{64.1} & \multicolumn{1}{l}{75.6} & \multicolumn{1}{l}{6.01} & \multicolumn{1}{l}{43.2} & \multicolumn{1}{l}{55.3} \\ \hline
% % Ours                                   & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{3.82} & \multicolumn{1}{l}{64.2} & \multicolumn{1}{l}{75.9} & \multicolumn{1}{l}{6.04} & \multicolumn{1}{l}{41.9} & \multicolumn{1}{l}{57.3} \\ \hline
% Ours                                   & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\ \hline
% \multirow{2}{*}{Speaker-Follower}      &                      & \checkmark            & \checkmark            & 3.88                 & 0.63                 & 0.71                 & 5.24                 & 0.50                 & 0.63                 \\
%                                       & \checkmark            & \checkmark            & \checkmark            & \textbf{3.08}                 & \textbf{0.70}                 & \textbf{0.78}                 & \textbf{4.83}                 & 0.55                 & 0.65                 \\
% \multirow{2}{*}{Ours (self-awareness)} &                      &                      &                      & 3.72                 & 0.63                 & 0.75                 & 5.98                 & 0.44                 & 0.58                 \\
%                                       &                      &                      & \checkmark            & 3.23                 & \textbf{0.70}                 & \textbf{0.78}                 & 5.04                 & \textbf{0.57}                 & \textbf{0.70}                 \\ \Xhline{2\arrayrulewidth}
% \end{tabular}
% \end{table}
% ====================================================================================

% ====================================================================================
% \begin{table}[t]
% \centering
% \small
% \tabcolsep=0.13cm
% \caption{
%     Ablation study showing the effect of each proposed method compared to the prior arts. All methods are using panoramic action space.
%     \textcolor{red}{remove full speaker-follower model with data augmentation?}
%     }
% \label{table:ablation-study-3}
% \begin{tabular}{cccccccccc}
% \Xhline{2\arrayrulewidth}
%                                       & Data                 & Pragmatic            & Beam                 & \multicolumn{3}{c}{Validation-Seen}                                & \multicolumn{3}{c}{Validation-Unseen}                              \\ \cline{5-10} 
%                                       & Augmentation         & Inference            & Search               & NE $\downarrow$ & SR $\uparrow$ & OSR $\uparrow$ & NE $\downarrow$ & SR $\uparrow$ & OSR $\uparrow$ \\ \hline
% \multirow{3}{*}{Speaker-Follower}                       &                      &                      &                      & 4.86                 & 0.52                 & 0.63                 & 7.07                 & 0.31                 & 0.41                \\
% &                      & \checkmark            & \checkmark            & 3.88                 & 0.63                 & 0.71                 & 5.24                 & 0.50                 & 0.63                 \\
%                                       & \checkmark            & \checkmark            & \checkmark            & \textbf{3.08}                 & \textbf{0.70}                 & \textbf{0.78}                 & \textbf{4.83}                 & 0.55                 & 0.65                 \\ \hline
% % Ours                                   & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{3.73} & \multicolumn{1}{l}{64.1} & \multicolumn{1}{l}{75.6} & \multicolumn{1}{l}{6.01} & \multicolumn{1}{l}{43.2} & \multicolumn{1}{l}{55.3} \\ \hline
% % Ours                                   & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{3.82} & \multicolumn{1}{l}{64.2} & \multicolumn{1}{l}{75.9} & \multicolumn{1}{l}{6.04} & \multicolumn{1}{l}{41.9} & \multicolumn{1}{l}{57.3} \\ \hline
% \multirow{2}{*}{Ours}                                   &  &  &  & 3.65 & 0.65 & 0.75 & 6.07 & 0.42 & 0.57 \\ 
% &                      &                      & \checkmark            & 3.66                 & 0.66                 & 0.76                 & 5.70                 & 0.49                 & 0.68                 \\ \hline
% % \multirow{2}{*}{Speaker-Follower}      &                      & \checkmark            & \checkmark            & 3.88                 & 0.63                 & 0.71                 & 5.24                 & 0.50                 & 0.63                 \\
% %                                       & \checkmark            & \checkmark            & \checkmark            & \textbf{3.08}                 & \textbf{0.70}                 & \textbf{0.78}                 & \textbf{4.83}                 & 0.55                 & 0.65                 \\
% \multirow{2}{*}{Ours (self-awareness)} &                      &                      &                      & 3.72                 & 0.63                 & 0.75                 & 5.98                 & 0.44                 & 0.58                 \\
%                                       &                      &                      & \checkmark            & 3.23                 & \textbf{0.70}                 & \textbf{0.78}                 & 5.04                 & \textbf{0.57}                 & \textbf{0.70}                 \\ \Xhline{2\arrayrulewidth}
% \end{tabular}
% \end{table}
% ====================================================================================

% % ====================================================================================
% \begin{table}[t]
% \centering
% \small
% \tabcolsep=0.15cm
% \renewcommand{\arraystretch}{1.2}
% \caption{
%     Ablation study showing the effect of each proposed components compared to the prior arts. All methods are using panoramic action space.
%     We implemented the model from Speaker-Follower~(\cite{fried2018speaker}) with panoramic action space as baseline.
%     % \protect\footnotemark.
%     }
% \label{table:ablation-study-4}
% \begin{tabular}{cccccccccccc}
% \Xhline{2\arrayrulewidth}
% &    & Positional & Self-     & Beam      & Data         & \multicolumn{3}{c}{Validation-Seen} & \multicolumn{3}{c}{Validation-Unseen} \\ \cline{7-12} 
% & \# & Encoding   & awareness & Search    & Augmentation & NE         & SR         & OSR       & NE          & SR         & OSR        \\ \hline
% Baseline &    &            &           &           &              & 4.36       & 0.54       & 0.68      & 7.22        & 0.27       & 0.39       \\ \hline
% \multirow{7}{*}{Ours}                                                 & 1  &            &           &           &              &            &            &           &             &            &            \\
% & 2  & \checkmark  &           &           &              & 3.65       & 0.65       & 0.75      & 6.07        & 0.42       & 0.57       \\
% & 3  & \checkmark  &  & \checkmark          &              & 3.66       & 0.66       & 0.76      & 5.70        & 0.49       & 0.68       \\ \cline{3-12}
% & 4  & \checkmark  & \checkmark &           &              & 3.72       & 0.63       & 0.75      & 5.98        & 0.44       & 0.58       \\
% & 5  & \checkmark  & \checkmark & \checkmark &              & 3.23       & 0.70       & \textbf{0.78}      & 5.04        & 0.57       & \textbf{0.70}       \\ \cline{3-12}
% & 6  & \checkmark  & \checkmark &           & \checkmark    & 3.22       & 0.67       & \textbf{0.78}      & 5.52        & 0.45       & 0.56   \\
% & 7  & \checkmark  & \checkmark & \checkmark & \checkmark    & \textbf{3.04}  & \textbf{0.71}  & \textbf{0.78} & \textbf{4.62}   & \textbf{0.58}  & 0.68  \\ \Xhline{2\arrayrulewidth}
% \end{tabular}
% \end{table}
% % ====================================================================================

% \footnotetext{Note that our results for this baseline are slightly higher on val-seen and slightly lower on val-unseen than those reported, due to differences in hyper-parameter choices. We thank the authors for communicating with us and providing details of the implementation.}

% ====================================================================================
% \begin{table}[t]
% \centering
% \small
% \tabcolsep=0.15cm
% \renewcommand{\arraystretch}{1.2}
% \caption{
%     Ablation study showing the effect of each proposed components compared to the prior arts. All methods are using panoramic action space.
%     *: we implemented the model from Speaker-Follower~(\cite{fried2018speaker}) with panoramic action space as baseline.
%     % \protect\footnotemark.
%     }
% \label{table:ablation-study-4}
% \begin{tabular}{ccccccccccc}
% \Xhline{2\arrayrulewidth}
% &     & Progress     & Beam      & Data         & \multicolumn{3}{c}{Validation-Seen} & \multicolumn{3}{c}{Validation-Unseen} \\ \cline{6-11} 
% & \#  & Monitor & Search    & Augmentation & NE $\downarrow$         & SR $\uparrow$         & OSR $\uparrow$      & NE $\downarrow$          & SR $\uparrow$        & OSR $\uparrow$       \\ \hline
% Baseline* &    &      &           &              & 4.36       & 0.54       & 0.68      & 7.22        & 0.27       & 0.39       \\ \hline
% % \multirow{7}{*}{Ours}                                                 & 1  &            &           &              &            &            &           &             &            &            \\
% \multirow{6}{*}{Ours} & 1  &           &           &              & 3.65       & 0.65       & 0.75      & 6.07        & 0.42       & 0.57       \\
% & 2  &  & \checkmark          &              & 3.66       & 0.66       & 0.76      & 5.70        & 0.49       & 0.68       \\ \cline{3-11}
% & 3  & \checkmark &           &              & 3.62       & 0.65       & 0.75      & 5.98        & 0.44       & 0.58       \\
% & 4  & \checkmark & \checkmark &              & 3.23       & 0.70       & \textbf{0.78}      & 5.04        & 0.57       & \textbf{0.70}       \\ \cline{3-11}
% & 5  & \checkmark &           & \checkmark    & 3.22       & 0.67       & \textbf{0.78}      & 5.52        & 0.45       & 0.56   \\
% & 6  & \checkmark & \checkmark & \checkmark    & \textbf{3.04}  & \textbf{0.71}  & \textbf{0.78} & \textbf{4.62}   & \textbf{0.58}  & 0.68  \\ \Xhline{2\arrayrulewidth}
% \end{tabular}
% \end{table}

% ====================================================================================
\begin{table}[b]
\centering
\small
\tabcolsep=0.15cm
\renewcommand{\arraystretch}{1.2}
\caption{
    Ablation study showing the effect of each proposed component compared to the prior art. All methods use a panoramic action space.
    *: we implemented the model from Speaker-Follower~\citep{fried2018speaker} with panoramic action space as baseline.
    % \protect\footnotemark.
    }
\label{table:ablation-study-4}
\begin{tabular}{ccccccccccc}
\Xhline{2\arrayrulewidth}
&     & Co-     & Progress      & Data         & \multicolumn{3}{c}{Validation-Seen} & \multicolumn{3}{c}{Validation-Unseen} \\ \cline{6-11} 
& \#  & Grounding & Monitor    & Augmentation & NE $\downarrow$         & SR $\uparrow$         & OSR $\uparrow$      & NE $\downarrow$          & SR $\uparrow$        & OSR $\uparrow$       \\ \hline
Baseline* &    &      &           &              & 4.36       & 0.54       & 0.68      & 7.22        & 0.27       & 0.39       \\ \hline
% \multirow{7}{*}{Ours}                                                 & 1  &            &           &              &            &            &           &             &            &            \\
\multirow{3}{*}{Ours} & 1  & \checkmark           &           &              & 3.65       & 0.65       & 0.75      & 6.07        & 0.42       & 0.57       \\
% & 2  & \checkmark  &           & \checkmark& 3.11       & 0.70       & \textbf{0.78}      & 5.84        & 0.45       & 0.54       \\
& 2  & \checkmark  & \checkmark          &              & 3.23       & 0.70       & \textbf{0.78}      & 5.04        & 0.57       & \textbf{0.70}       \\
& 3  & \checkmark & \checkmark & \checkmark & \textbf{3.04}  & \textbf{0.71}  & \textbf{0.78} & \textbf{4.62}   & \textbf{0.58}  & 0.68  \\ \Xhline{2\arrayrulewidth}
% & 4  & \checkmark & \checkmark & \checkmark             & 3.23       & 0.70       & \textbf{0.78}      & 5.04        & 0.57       & \textbf{0.70}       \\ 
% & 5  & \checkmark & \checkmark & \checkmark    & 3.22       & 0.67       & \textbf{0.78}      & 5.52        & 0.45       & 0.56   \\
% & 6  & \checkmark & \checkmark & \checkmark    & \textbf{3.04}  & \textbf{0.71}  & \textbf{0.78} & \textbf{4.62}   & \textbf{0.58}  & 0.68  \\ \Xhline{2\arrayrulewidth}
\end{tabular}
\end{table}
